Oscillation frequencies for 35 \Kepler solar-type planet-hosting stars using Bayesian techniques and machine learning

\Kepler has revolutionised our understanding of both exoplanets and their host stars. Asteroseismology is a valuable tool in the characterisation of stars and \Kepler is an excellent observing facility to perform asteroseismology. Here we select a sample of 35 \Kepler solar-type stars which host transiting exoplanets (or planet candidates) with detected solar-like oscillations. Using available \Kepler short cadence data up to Quarter 16 we create power spectra optimised for asteroseismology of solar-type stars. We identify modes of oscillation and estimate mode frequencies by ``peak bagging'' using a Bayesian MCMC framework. In addition, we expand the methodology of quality assurance using a Bayesian unsupervised machine learning approach. We report the measured frequencies of the modes of oscillation for all 35 stars and frequency ratios commonly used in detailed asteroseismic modelling. Due to the high correlations associated with frequency ratios we report the covariance matrix of all frequencies measured and frequency ratios calculated. These frequencies, frequency ratios, and covariance matrices can be used to obtain tight constraint on the fundamental parameters of these planet-hosting stars.

==> Results/11295426_correl.tex <==
\begin{figure}
   \includegraphics[width=80mm]{COR/cor_11295426.png}
   \caption{Correlation matrix of all frequencies and ratios for KIC 11295426.  The grid represents the matrix and hence the identity elements are all correlation 1.0.  The matrix is constructed so that frequencies and ratios are grouped separately.  If each matrix element is labelled $[i,j]$ then the first set of $i$ contains the mode frequencies, the second set contains the $r_{010}$, and the final set the $r_{02}$.}   \label{fig::cor_11295426}\end{figure}

==> Results/11295426_freqs.tex <==
\begin{figure}
   \includegraphics[width=80mm]{PSD/psd_11295426.png}
   \includegraphics[width=80mm]{ED/ed_11295426.png}
   \caption{Power spectrum and echelle diagram for KIC 11295426.  Top: Power spectrum with data in grey smoothed over $3 \; \rm \mu Hz$ and best model in black.  Bottom: Echelle diagram with power in grey-scale.  Both: Mode frequencies are marked as: radial modes with red circles; dipole modes with green diamonds; quadrapole modes with blue squares; and octopole modes with yellow pentagons.}   \label{fig::11295426}\end{figure}

==> Results/11295426_ratios.tex <==
\begin{figure}
   \includegraphics[width=80mm]{RAT/rall_11295426.png}
   \caption{Ratios and $67 \%$ confidence intervals as a function of frequency for KIC 11295426.}   \label{fig::rat_11295426}\end{figure}

==> Results/3632418_results.tex <==
\begin{figure*}
   \includegraphics[width=80mm]{PSD/psd_3632418.png}
   \includegraphics[width=80mm]{ED/ed_3632418.png}
   \caption{Power spectrum and echelle diagram for 3632418.}\end{figure*}

==> Results/7199397_correl.tex <==
\begin{figure}
   \includegraphics[width=80mm]{COR/cor_7199397.png}
   \caption{Correlation matrix for 7199397.  Top left box is freqs, middle is r02, and bottom right is r010.}\end{figure}

==> Results/7199397_ratios.tex <==
\begin{figure}
   \includegraphics[width=80mm]{RAT/rall_7199397.png}
   \caption{Ratios as a function of frequency for 7199397.}\end{figure}

==> Results/8684730_correl.tex <==
\begin{figure}
   \includegraphics[width=80mm]{COR/cor_8684730.png}
   \caption{Correlation matrix of all frequencies and ratios for KIC 8684730.  The grid represents the matrix and hence the identity elements are all correlation 1.0.  The matrix is constructed so that frequencies and ratios are grouped separately.  If each matrix element is labelled $[i,j]$ then the first set of $i$ contains the mode frequencies, the second set contains the $r_{010}$, and the final set the $r_{02}$.}   \label{fig::cor_8684730}\end{figure}

==> Results/8684730_ratios.tex <==
\begin{figure}
   \includegraphics[width=80mm]{RAT/rall_8684730.png}
   \caption{Ratios and $67 \%$ confidence intervals as a function of frequency for KIC 8684730.}   \label{fig::rat_8684730}\end{figure}

==> targets1.tex <==
\begin{table}
   \label{tab::basic}
   \caption{Targets and basic info.}
   \begin{tabular}{cccccc}
   \hline
   \hline
   KOI & KIC & $\nu_{\rm max}$ & $\Delta \nu$ & $T_{\rm eff}$ \\
   & & $\rm \mu Hz$ & $\rm \mu Hz$ & K \\
   \hline
   268 & 3425851 & 1912 & 94 & $6343 \pm 85$ \\
   69 & 3544595 & 3021 & 147 & $5669 \pm 75$ \\
   975 & 3632418 & 1150 & 64 & $6305 \pm 50$ \\
   280 & 4141376 & 2909 & 225 & $6134 \pm 91$ \\
   281 & 4143755 & 1434 & 74 & $5622 \pm 106$ \\
   244 & 4349452 & 2089 & 99 & $6270 \pm 79$ \\
   108 & 4914423 & 1641 & 82 & $5845 \pm 88$ \\
   123 & 5094751 & 1817 & 90 & $5952 \pm 75$ \\
   85 & 5866724 & 1864 & 90 & $6169 \pm 50$ \\
   285 & 6196457 & 1377 & 80 & $5871 \pm 94$ \\
   3158 & 6278762 & 4278 & 181 & $5046 \pm 74$ \\
   41 & 6521045 & 1495 & 76 & $5825 \pm 75$ \\
   75 & 7199397 & 640 & 40 & $5824 \pm 50^{\star}$ \\
   269 & 7670943 & 1871 & 91 & $6463 \pm 110$ \\
   274 & 8077137 & 1299 & 69 & $6105 \pm 100$ \\
   260 & 8292840 & 1966 & 94 & $6205 \pm 100$ \\
   122 & 8349582 & 1617 & 84 & $5699 \pm 74$ \\
   245 & 8478994 & 4421 & 181 & $5417 \pm 75$ \\
   370 & 8494142 & 1140 & 62 & $6144 \pm 106$ \\
   5 & 8554498 & 1170 & 74 & $5945 \pm 60$ \\
   319 & 8684730 & 950 & 81 & $5880 \pm 87^{\dagger}$ \\
   42 & 8866102 & 2022 & 97 & $6325 \pm 75$ \\
   974 & 9414417 & 1137 & 64 & $6253 \pm 75$ \\
   288 & 9592705 & 996 & 54 & $6174 \pm 92$ \\
   1925 & 9955598 & 3545 & 153 & $5460 \pm 75$ \\
   263 & 10514430 & 1280 & 68 & $5784 \pm 98$ \\
   275 & 10586004 & 1335 & 71 & $5770 \pm 83$ \\
   2 & 10666592 & 1092 & 60 & $6350 \pm 80$ \\
   1612 & 10963065 & 2165 & 104 & $6104 \pm 74$ \\
   276 & 11133306 & 2213 & 105 & $5982 \pm 82$ \\
   246 & 11295426 & 2151 & 103 & $5793 \pm 74$ \\
   277 & 11401755 & 1226 & 67 & $5960 \pm 80$ \\
   262 & 11807274 & 1471 & 77 & $6225 \pm 75$ \\
   7 & 11853905 & 1493 & 77 & $5781 \pm 76$ \\
   72 & 11904151 & 2418 & 112 & $5647 \pm 74$ \\
   \hline
   \end{tabular}
\end{table}

